VietMed: A Dataset and Benchmark for Automatic Speech Recognition of Vietnamese in the Medical Domain

Due to privacy restrictions, there's a shortage of publicly available speech recognition datasets in the medical domain. In this work, we present VietMed - a Vietnamese speech recognition dataset in the medical domain comprising 16h of labeled medical speech, 1000h of unlabeled medical speech and 1200h of unlabeled general-domain speech. To our best knowledge, VietMed is by far the world's largest public medical speech recognition dataset in 7 aspects: total duration, number of speakers, diseases, recording conditions, speaker roles, unique medical terms and accents. VietMed is also by far the largest public Vietnamese speech dataset in terms of total duration. Additionally, we are the first to present a medical ASR dataset covering all ICD-10 disease groups and all accents within a country. Moreover, we release the first public large-scale pre-trained models for Vietnamese ASR, w2v2-Viet and XLSR-53-Viet, along with the first public large-scale fine-tuned models for medical ASR. Even without any medical data in unsupervised pre-training, our best pre-trained model XLSR-53-Viet generalizes very well to the medical domain by outperforming state-of-the-art XLSR-53, from 51.8% to 29.6% WER on test set (a relative reduction of more than 40%). All code, data and models are made publicly available: https://github.com/leduckhai/MultiMed/tree/master/VietMed.

==> content.tex <==
% Don't add the documentclass, usepackage, etc here. that goes into main.tex!
% new packages as well

\title{VietMed: A Dataset and Benchmark for \\Automatic  Speech Recognition of Vietnamese \\in the Medical Domain}

\name{Khai Le-Duc$^{*}$} 


%\address{Affiliation1, Affiliation2, Affiliation3 \\
%         Address1, Address2, Address3 \\
%         author1@xxx.yy, author2@zzz.edu, author3@hhh.com\\
%         \{author1, author5, author9\}@abc.org\\}
         

\address{
University of Toronto, Canada\\
duckhai.le@mail.utoronto.ca}


\abstract{
Due to privacy restrictions, there's a shortage of publicly available speech recognition datasets in the medical domain.
In this work, we present \textit{VietMed} - a Vietnamese speech recognition dataset in the medical domain comprising 16h of labeled medical speech, 1000h of unlabeled medical speech and 1200h of unlabeled general-domain speech.
To our best knowledge, \textit{VietMed} is by far the world's largest public medical speech recognition dataset in 7 aspects: total duration, number of speakers, diseases, recording conditions, speaker roles, unique medical terms and accents.
\textit{VietMed} is also by far the largest public Vietnamese speech dataset in terms of total duration.
Additionally, we are the first to present a medical ASR dataset covering all ICD-10 disease groups and all accents within a country.
Moreover, we release the first public large-scale pre-trained models for Vietnamese ASR, \textit{w2v2-Viet} and \textit{XLSR-53-Viet}, along with the first public large-scale fine-tuned models for medical ASR.
Even without any medical data in unsupervised pre-training, our best pre-trained model \textit{XLSR-53-Viet} generalizes very well to the medical domain by outperforming state-of-the-art \textit{XLSR-53}, from  51.8\% to 29.6\% WER on test set (a relative reduction of more than 40\%).
All code, data and models are made publicly available \href{https://github.com/leduckhai/MultiMed/tree/master/VietMed}{here}.
\\ \newline \Keywords{medical speech recognition, dataset, semi-supervised learning}} 


\begin{document}
\pagenumbering{arabic}
%\pagestyle{fancy}
%\fancyhf{}
%\fancyhf[rh]{\thepage}
%\renewcommand\headrulewidth{0pt}
\maketitleabstract

\def\thefootnote{(*)}\footnotetext{Work done during the bachelor thesis at Lehrstuhl Informatik 6 - Machine Learning and Human Language Technology Group, RWTH Aachen University, Germany}\def\thefootnote{\arabic{footnote}}

\section{Introduction}

Machine learning models require large amounts of training data.
However, the scarcity of language resources for Vietnamese and especially for the medical domain has been hindering the advancement of corresponding automatic speech recognition (ASR) systems.
Also, the lack of publicly available speech datasets and models in these domains has led to difficulties in reproducing experiments.

Recently, research efforts have been directed towards ASR tasks in the medical field, such as the works \cite{luescher2022:hykist, vieting2023efficient} focused on the development of hybrid ASR systems to transcribe multilingual telephone speech data from patient-physician conversations.
Besides, the works \cite{edwards2017medical, chiu18_interspeech} tackled difficult acoustic conditions and the absence of domain-specific data. 
Nevertheless, none of these studies released their own datasets or pre-trained models.

Out of the limited number of public medical speech datasets we identified, to the best of our knowledge, one of them offers a total of 8 hours of English speech data; however, the dataset's quality is low, as indicated by the authors on their webpage\footnote{https://www.kaggle.com/datasets/paultimothymooney/medical-speech-transcription-and-intent}, where they mentioned issues such as incorrect labels and audio files. 
The second public English medical speech dataset \cite{fareez2022dataset} comprises simulated data, with a predominant focus on respiratory diseases.
This situation restricts investigations to a single disease topic, hindering researchers from exploring experiments related to other medical conditions. 
Also, as pointed out by the authors, this dataset collected speech exclusively from the West England population, which might hurt generalizability to other accents.

Regarding Vietnamese ASR, to the best of our knowledge, there are currently no public large-scale pre-trained models that are peer-reviewed and reproducible\footnote{Several pre-trained models for Vietnamese ASR are available on HuggingFace and GitHub, but none of them have undergone peer review. Their results are self-reported, and we were unable to reproduce them.}.
The \textit{XLSR-53} model \cite{conneau21_interspeech}, was unsupervised pre-trained on 56k hours of 53 languages, but it includes only 200 hours of Vietnamese data. 
Therefore, the constrained performance when fine-tuning the \textit{XLSR-53} model on Vietnamese is conceivable \cite{bachelorthesis}. 

To handle the concerns above, we present a high-quality dataset for Vietnamese medical speech recognition. 
To the best of our knowledge, \textit{VietMed} is by far the world's largest public medical speech dataset in terms of total duration, number of speakers, diseases, recording conditions, speaker roles, unique medical terms and accents. 
Also, \textit{VietMed} is by far the largest public Vietnamese speech dataset in terms of total duration.
Moreover, \textit{VietMed} is the first medical ASR dataset covering all ICD-10 disease groups and all accents within a country.
We then empirically evaluate baseline models on our dataset. 
Our key contributions are:
\begin{itemize}
    \item We present \textit{VietMed} dataset, which includes 16 hours of labeled medical speech, 1000 hours of unlabeled medical speech and 1200 hours of unlabeled general-domain speech.
    \item We release the first public large-scale pre-trained models for Vietnamese ASR, which are peer-reviewed and reproducible.   
    \item We release the first public large-scale fine-tuned models for medical ASR. 
\end{itemize}

Given the transferability of medical terms across languages at some degree, our aim is to contribute to future research in medical ASR for other languages.
All code, data and models are published online\footnote{\url{https://github.com/leduckhai/MultiMed/tree/master/VietMed}}$^{,}$\footnote{https://github.com/rwth-i6/returnn-experiments}.


\section{Data}
\textit{\textit{VietMed}} data comprises of 3 sets, namely \textit{VietMed-L} for labeled medical speech, \textit{VietMed-U} for unlabeled medical speech, and \textit{Viet-U} for unlabeled general domain speech.
We then split \textit{VietMed-L} into 3 subsets, train (\textit{VietMed-Train}), dev (\textit{VietMed-Dev}) and test (\textit{VietMed-Test}) with duration being 5 hours, 5 hours, and 6 hours respectively, avoiding speaker overlap between the train, dev and test sets.

\subsection{Metadata}
\input{tabs_and_figs/meta_data}

We saved all the metadata information to files named Metadata\_labeled.xlsx and Medical\_terms.txt.
As shown in Table \ref{meta_data}, we designed metadata in a way that can support multiple tasks apart from ASR, for example: speaker recognition, keyword recognition, or accent recognition.

\subsection{Data Collection}
We first legally crawled audio data from YouTube under Fair Use Policies\footnote{https://support.google.com/youtube/answer/9783148}$^{,}$\footnote{https://www.copyright.gov/fair-use/} (Details of Fair Use and Consent are in the Appendix).
We manually removed non-speech elements like music, noise, long silences, and any parts that could reveal speaker identities.
Specifically, we removed speaker names, locations where they live, organizations where they work, personal contacts (phone numbers, emails, etc.), personal identifier (date of birth, bank account, id number, etc.), etc.
We converted MP3 audio files to 8kHz wav format, creating 10-30 second segments for \textit{VietMed-U} and \textit{Viet-U}, and <10 second segments for \textit{VietMed-L}. 
Also, we encoded segment names, retaining only ICD-10 code tags to enhance privacy.
Finally, we shuffled all segments of \textit{VietMed-U} and \textit{Viet-U}, making about 500k meaningless segments. 
The purpose here is to prevent immoral users from concatenating segments into meaningful conversations to learn more about speakers.

\subsection{Annotation Process}
Manual annotation of medical spontaneous speech is challenging for humans \cite{edwards2017medical}. 
Annotators may produce varying transcripts. 
Also, applying the fully automated approach \cite{gigaspeech2021} requires large-scale ASR models, which are unavailable in the medical domain and suffer from low quality due to limited human supervision.
We therefore implemented a computer-assisted workflow for medical annotation, outlined as follows:
\begin{enumerate}
    \item We initially gathered transcripts generated by YouTube.
    \item A native Vietnamese with a Biomedical Engineering degree corrected the automatically generated transcripts manually.
    This reduced annotation time by 70\% and improved transcript quality, as it could address issues like stuttering words and speaking rate variations common in real-world conversations.
    \item Another native Vietnamese independently annotated using the same approach.
    \item The resulting two computer-assisted annotation versions were merged and compared. Segments with large differences were excluded.
    \item Finally, we divided the merged transcripts into 3 small validation subsets, where three other Vietnamese with medical backgrounds assessed quality  through manual annotation without assistance by automatic transcription. 
    We then merged the computer-assisted and non-computer-assisted versions as in step 4.
\end{enumerate}

Detailed concerns about the noisy speech in our dataset are shown in the Appendix.

\subsection{Data Statistics}


\input{tabs_and_figs/data_stats}

\subsubsection{Labeled Medical Data \textit{VietMed-L}}
In Table \ref{data_stats}, \textit{VietMed-L} contains 16 hours of annotated audio, surpassing other private medical ASR datasets \cite{medisco, chung-etal-2021-data}.
Also, \textit{VietMed-L} has a much higher number of speakers and unique medical terms.
Unlike most datasets that only use simulated scenarios \cite{luescher2022:hykist, fareez2022dataset}, \textit{VietMed-L} captures real-life situations across 8 recording conditions, including telephone (e.g. telemedicine), lectures (e.g. in university hospitals), news (e.g. in medical centers), audiobooks (e.g. medical textbooks), where 85\% of the content is spontaneous speech.
Additionally, we include speech from various roles such as lecturers, hosts, broadcasters, beyond just doctors and patients. 
Furthermore, we ensure diversity by gathering 6 accents representing all regions.

\begin{figure*}[!ht]
\begin{center}
\includegraphics[scale=0.4]{tabs_and_figs/icd_accent_labeled_medical.png} 
\caption{Distribution of ICD-10 codes and accents in \textit{VietMed-L}.}
\label{icd_accents_gender_labeled_medical}
\end{center}
\end{figure*}

In Figure \ref{icd_accents_gender_labeled_medical}, rather than primarily focusing on the respiratory disease group (J00-J99) as in \cite{fareez2022dataset}, \textit{VietMed-L} has data from 22/22 disease groups as per World Health Organization (WHO)'s ICD-10 code\footnote{https://www.icd10data.com/ICD10CM/Codes}, supporting the dataset's generalizability.
Also, the accents closely match the real accent  distribution\footnote{https://www.gso.gov.vn/en/population/} (see Table \ref{list_of_regions_vietnam} in the Appendix), and the male/female ratio (54.7\%-45.3\%) is quite balanced.

\subsubsection{Unlabeled Medical Data \textit{VietMed-U}}
In Table \ref{data_stats}, we collected \textit{VietMed-U} in a manner similar to \textit{VietMed-L}, assuring a comparable generalizability as in Figure \ref{icd_accents_gender_labeled_medical}.
Distribution of ICD-10 codes and accents is in Figure \ref{icd_unlabeled_medical} and Figure \ref{accents_unlabeled_medical} of the Appendix.

\subsubsection{Unlabeled General Domain Data \textit{Viet-U}}
\input{tabs_and_figs/unlabeled_general_stats}

In real world, audiobooks are typically recorded using major Northern and Southern accents.
In Table \ref{unlabeled_general_stats}, statistics of \textit{Viet-U} is shown.

\input{tabs_and_figs/LM_results}

\subsection{Extra Text Data \textit{ExtraText}}
In Table \ref{LM_results}, besides \textit{VietMed-Train} for language model (LM), we used extra text data \textit{ExtraText} to gain lower PPLs. 
Sources are: 
VIVOS\footnote{http://ailab.hcmus.edu.vn/vivos} \cite{vivos_dataset}, BABEL\footnote{https://www.iarpa.gov/research-programs/babel}, CommonVoice\footnote{https://commonvoice.mozilla.org/} \cite{commonvoice_dataset}, FOSD\footnote{https://www.kaggle.com/datasets/thinh127/fpt-open-speech-dataset-fosd-vietnamese} \cite{FOSD_vietnamese_dataset}, VNTC-Health\footnote{https://github.com/duyvuleo/VNTC}, VLSP 2020\footnote{https://vlsp.org.vn/}, ViHealthBERT-FAQ \cite{vihealthbert} and PhoNER-Covid19 \cite{PhoNER_COVID19}.

\subsection{Lexicon}
We used the BABEL project's seed lexicon and augmented it with either \textit{VietMed-Train} or \textit{VietMed-Train} + \textit{ExtraText}.
Using the toolkit Sequitur Grapheme-To-Phoneme\footnote{https://github.com/sequitur-g2p/sequitur-g2p} \cite{G2P_toolkit} - the conversion tool on these pronunciation lexica, the seed lexicon was extended, creating the lexica for training.

\section{Experimental Setups}
For language modelling and initial Gaussian Mixture - Hidden Markov Model (GM-HMM), we followed the same setups and hyperparameters as in \cite{luescher2022:hykist}.
The acoustic model labels were generalized triphone states obtained by classification and regression trees with 4501 labels.
For unsupervised wav2vec 2.0 training \cite{facebook2020wav2vec2} and fine-tuning, we used the same vanilla setups and hyperparameters in \cite{bachelorthesis}.
All models had 118M parameters including 7 CNN layers and 8 Transformer layers.
The last CNN layer had a stride halved for the 8kHz data.
We then chose the pre-training epoch to fine-tune with Framewise Cross-Entropy (fCE) loss that led to the best WERs on dev.
The SpecAugment \cite{park2019specaugment} was used during 33 fine-tuning epochs.

We used RETURNN \cite{zeyer2018returnn} for supervised training and Fairseq \cite{facebook2019fairseq} for unsupervised wav2vec 2.0 training. 
Decoding was performed with RASR \cite{rybach2011rasr}. 
Fairseq models were converted to RETURNN models with our PyTorch-to-RETURNN toolkit\footnote{https://github.com/rwth-i6/pytorch-to-returnn}.


\section{Experimental Results}

\subsection{Language Model}
In Table \ref{LM_results}, augmenting the seed lexicon with only \textit{VietMed-Train} to train \textit{VietMed-Train}+\textit{ExtraText} for LM yields the best PPLs.

\subsection{GM-HMM Alignments}
\input{tabs_and_figs/gmm_hmm_results}
In Table \ref{gmm_hmm_results}, understanding that WER isn't always a precise metric for alignment quality assessment, we found that WER of SAT was quite similar to SAT+VTLN. 
Therefore, we chose SAT alignments as input for hybrid wav2vec 2.0 training to bypass some steps in GM-HMM process.

\subsection{Hybrid wav2vec 2.0 Baselines}
\input{tabs_and_figs/dnn_hmm_results}
As shown in Table \ref{dnn_hmm_results}, training from scratch did not converge, possibly due to the limited 5-hour fine-tuning data.
\textit{XLSR-53} is a state-of-the-art model pre-trained on 56k hours of 53 languages.
Fine-tuning \textit{XLSR-53} on \textit{VietMed-Train} helped reduce  WER from 52.6\% to 45.2\% on \textit{VietMed-Dev}.
Our \textit{w2v2-Viet} model was competitive to \textit{XLSR-53} despite using 46 times less data for pre-training.
We obtained further improvements by applying our \textit{XLSR-53-Viet} model, which reduced WERs to 26.8\% and 29.6\% on dev and test set respectively, equivalent to relative WERR of 41.8\% compared to the  \textit{XLSR-53} model.
In both our models, we didn't adapt the in-domain data \textit{VietMed-U} during the unsupervised pre-training, although we believed doing so could further enhance WERs and we leave it for future work.

\section{Conclusion}
In this work, we present \textit{VietMed} - a medical speech recognition dataset for Vietnamese.
We introduce a high-quality annotation approach for medical ASR dataset that saves 70\% of time.
Also, we outline our work on creating a LM with acceptable PPL and a compact size.
Finally, our best pre-trained model \textit{XLSR-53-Viet} outperforms the vanilla state-of-the-art \textit{XLSR-53} by reducing WERs from 51.8\% to 29.6\% WER on test set (a relative reduction of more than 40\%) without using any medical data in unsupervised pre-training.

\newpage

\section{Acknowledgements}
This work was partially supported by the project HYKIST funded by the German Federal Ministry of Health on the basis of a decision of the German Federal Parliament (Bundestag) under funding ID ZMVI1-2520DAT04A.

To our best knowledge, this is the very first time in history that the world's largest dataset came from Vietnam.
We thank Minh-Nghia Phan, Peter Vieting, Robin Schmitt, Moritz Gunz, Julian Dierkes for their precious assistance in experimental setups.

We also appreciate Christoph Lüscher, Ralf Schlüter, Hermann Ney for their valuable feedback on this work.

\newpage
%\nocite{*}

\section{Bibliographical References}\label{sec:reference}

\bibliographystyle{lrec-coling2024-natbib}
\bibliography{lrec-coling2024-example}

\include{suppl_material.tex}


\end{document}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

